On the Optimization of Approximate Control Variates with Parametrically Defined Estimators

Multi-model Monte Carlo methods, such as multi-level Monte Carlo (MLMC) and multifidelity Monte Carlo (MFMC), allow for efficient estimation of the expectation of a quantity of interest given a set of models of varying fidelities. Recently, it was shown that the MLMC and MFMC estimators are both instances of the approximate control variates (ACV) framework [Gorodetsky et al. 2020]. In that same work, it was also shown that hand-tailored ACV estimators could outperform MLMC and MFMC for a variety of model scenarios. Because there is no reason to believe that these hand-tailored estimators are the best among a myriad of possible ACV estimators, a more general approach to estimator construction is pursued in this work. First, a general form of the ACV estimator variance is formulated. Then, the formulation is utilized to generate parametrically-defined estimators. These parametrically-defined estimators allow for an optimization to be pursued over a larger domain of possible ACV estimators. The parametrically-defined estimators are tested on a large set of model scenarios, and it is found that the broader search domain enabled by parametrically-defined estimators leads to greater variance reduction.

==> formulation.tex <==
\section{Formulation}\label{sec:formulation}
In this section a general form of the approximate control variate framework (ACV) is explored.  As discussed in the work of \cite{gorodetsky}, the ACV framework provides a unifying structure with which to view several existing methods in the literature.  The framework outlined in that work is further extended here to enable creation of parametrically defined ACV estimators.  Two new generalized ACV estimators are then derived, while showing that existing ACV methodologies are specific instances of these estimators.


\subsection{Approximate Control Variate Estimation}
Let $(\Omega, \mathcal{F}, \mathcal{P})$ be a probability space and  %<- I dont know what this is but its at the beginning of their formulation?
 let $\{Q_0, Q_1, ..., Q_M\}$ be a set of $M + 1$ mappings $Q_i : \mathbb{R}^d \rightarrow \mathcal{Q}_i \subset  \mathbb{R}$ from vector-valued inputs to scalar outputs.  These mappings will henceforth be referred to as models. The primary goal of the ACV framework is to estimate the mean of $Q_0$ (\ie $\mu_0 = \E[Q_0]$) using a set of $N$ samples $z = \{z^{(0)}, z^{(1)}, ... z^{(N)} \}$ of the input random variables and $M$ correlated models $\{Q_1, Q_2..., Q_M\}$.  Since $Q_0$ model holds particular significance it is referred to as the high fidelity model, the remaining models are referred to as low fidelity models.  As derived in \cite{gorodetsky} the general form of the ACV estimator is \footnote{As in the referenced work, attention is restricted to the linear control variate case}:
\begin{equation}
\tilde {Q}(\vec{\alpha}, z, \mathcal{A}) = \hat Q_0 (z_0) + \sum_{i=1}^M\alpha_i \left( \hat Q_i (z^*_i) -  \hat Q_i (z_i) \right) 
\label{eq:acv}
\end{equation}
where $\vec{\alpha} = \{ \alpha_1, \alpha_2, .., \alpha_M \} $ are the control variate weights and $z_0$, $z_i$, and $z^*_i$ are subsets of $z$ such that their union is $z$: \ie $z_0 \cup z^*_1 \cup z_1 \cup ... \cup z^*_M \cup z_M = z$.  Note that the subsets can, and usually do, overlap such that $z_i, z^*_i \cap z_j, z^*_j \neq \varnothing$.  $a$ represents the information associated with the allocation of $z$ into its subsets $z_0$, $z_i$, and $z^*_i$.  Specifically, $\mathcal{A}$ contains the number of samples in $z$, the number of samples in each subset, the number of samples in the intersections of pairs of subsets, and the number of samples in the union of pairs of subsets: $N$, $N_i$, $N_{i\cap j}$, and $N_{i\cup j}$, respectively.  Note that $\mathcal{A}$ does not contain the values of the samples themselves. In the above equation, $\hat Q_k(z_\ell)$ is the Monte Carlo (MC) estimator for $\E[Q_k]$ using samples $z_\ell$:
\begin{equation}
\hat Q_k (z_\ell) = \frac{1}{N_\ell} \sum_i^{N_\ell} Q_k\left(z_\ell^{(i)} \right)
\end{equation}
where $N_\ell$ is the number of samples in $z_\ell$.  Given that model $Q_k$ has bounded variance $\Var[Q_k]$, the variance of the MC estimator is
\begin{equation}
\Var[\hat Q_k (z_\ell)] = \frac{1}{N_\ell} \Var[Q_k]
\label{eq:mc_var}
\end{equation}
as as $N_\ell \rightarrow \infty$.  Note that this variance is a function of the sample allocation (containing $N_\ell$) and the model statistics (\ie $\Var[Q_k]$) and not a function of samples themselves.

Because \eref{eq:acv} is an unbiased estimator, the minimum variance estimator is the one with minimal error.  By first organizing \eref{eq:acv} in vector form:
\begin{equation}
\tilde {Q}(\vec{\alpha}, z, \mathcal{A}) =  \hat Q_0 (z_0) + \sum_{i=1}^M\alpha_i \Delta_i(z^*_i, z_i) = \hat Q_0 + \vec{\alpha}^T \vec{\Delta}
\end{equation}
Where $\vec{\Delta} = \{ \Delta_1(z^*_1, z_1), ..., \Delta_M(z^*_M, z_M) \}$ and $\Delta_i(z^*_i, z_i) =\hat Q_i (z^*_i) -  \hat Q_i (z_i)$.  The variance of the estimator can be written:
\begin{equation}
\Var[\tilde Q(\vec{\alpha}, z, \mathcal{A})] = \Var[\hat Q_0] +\vec{\alpha}^T(\Cov[\vec{\Delta}, \vec{\Delta}]) \vec{\alpha} + 2\vec{\alpha}^T \Cov[\vec{\Delta}, \hat Q_0]
 \label{eq:acv_est_var}
\end{equation}
Noting that the explicit dependence on $z^*_i, z_i$ of the terms on the right hand side have been dropped for simplification of notation.
The optimal control variate weights, corresponding to a minimum variance for a given $z$ and $\mathcal{A}$ are then
\begin{align}
\begin{split}
 \vec{\alpha}_{opt}(z, \mathcal{A}) &= \arg \min_{\vec{\alpha}} \Var[\tilde {Q}(\vec{\alpha}, z, \mathcal{A})] \\
 &= -\Cov[\vec{\Delta}, \vec{\Delta}]^{-1}\Cov[\vec{\Delta}, \hat Q_0]
 \end{split}
 \label{eq:opt_alpha}
\end{align}
Inserting \eref{eq:opt_alpha} into \eref{eq:acv_est_var} gives the variance of the $\alpha$-optimal ACV estimator:
\begin{equation}
\Var[\tilde Q^{\vec{\alpha}_{opt}}(z, \mathcal{A})] = \Var[\hat Q_0] - \Cov[\vec{\Delta}, \hat Q_0]^T \Cov[\vec{\Delta}, \vec{\Delta}]^{-1} \Cov[\vec{\Delta}, \hat Q_0]
 \label{eq:acv_est_var_alpha_optimal}
\end{equation}
See \aref{app:acv_var_alpha} for the complete derivations of \eqs{eq:acv_est_var}{eq:opt_alpha} as first detailed in the work of Gorodetsky et al.\ref{gorodetsky2018}.  Similar to the MC estimator variance, the variance of the ACV estimator and $\vec{\alpha}_{opt}$ do not depend on $z$.   Proof of this comes from the further development of the relationship of ACV estimator variance and $\mathcal{A}$.

Since the ACV estimator variance in \eref{eq:acv_est_var} is a function of the scalar $\Var[\hat Q_0]$, the matrix $\Cov[\vec{\Delta}, \vec{\Delta}]$, and the vector $\Cov[\vec{\Delta}, \hat Q_0]$, each of these quantities needs to be related to $\mathcal{A}$.  Using \eref{eq:mc_var}, the first of these terms is related to $\mathcal{A}$ as $\Var[\hat Q_0] = N_0^{-1}\Var[Q_0]$.  The remaining two terms have previously only been linked to $\mathcal{A}$ for specific sample allocation strategies.  For example, the estimators developed in the work of Gorodetsky et al. \cite{gorodetsky2008} take the following form:
\begin{align}
\Cov[\vec{\Delta}, \vec{\Delta}] &= \mathbf{F}(\mathcal{A}) \circ \mathbf{C} \\
\Cov[\vec{\Delta}, \hat Q_0] &= \text{diag}(\mathbf{F}(\mathcal{A})) \circ \mathbf{c}
\end{align}
where $\mathbf{C} \in \mathbb{R}^{M\text{x}M}$ is the covariance matrix among low fidelity models $\{Q_1, ..., Q_M\}$ and $\mathbf{c} \in \mathbb{R}^M$ is the covariance vector of the low fidelity models $\{Q_1, ..., Q_M\}$ with the high fidelity model $Q_0$.  A matrix $\mathbf{F} \in \mathbb{R}^{M\text{x}M}$ was derived as a function of $\mathcal{A}$ for each of the specific sample allocation strategies in that work.  

A more general, albeit structurally similar relationship, can be derived based on the covariance of MC estimators.  The covariance of two MC estimators is:
\begin{equation}
\Cov[\hat Q_i (z_j), \hat Q_k (z_\ell)] = \frac{N_{j \cap \ell}}{N_jN_\ell}Cov\left[Q_i , Q_k \right]
\label{eq:cov_mc_estimators}
\end{equation}
where $N_{j \cap \ell}$ is the number of samples in the intersection of $z_j$ and $z_\ell$. The full proof of which is located in \aref{app:cov_mc_estimators}.  Focusing first on the elements of $\Cov[\vec{\Delta}, \hat Q_0]$, their general form can be derived from the definition of $\vec{\Delta}$, the covariance of sums, and \eref{eq:cov_mc_estimators}:
\begin{equation}
\begin{split}
\Cov[\vec{\Delta}_i, \hat Q_0] &= \Cov[\hat Q_i(z^*_i) - \hat Q_i(z_i), \hat Q_0(z_0)]\\
&= \Cov[\hat Q_i(z^*_i), \hat Q_0(z_0)] - \Cov[\hat Q_i(z_i), \hat Q_0(z_0)]\\
&= \frac{N_{i* \cap 0}}{N_{i*}N_0}\Cov[Q_i , Q_0 ] - \frac{N_{i \cap 0}}{N_{i}N_0}\Cov[Q_i , Q_0 ]\\
&= \left(\frac{N_{i* \cap 0}}{N_{i*}N_0} - \frac{N_{i \cap 0}}{N_{i}N_0} \right) \Cov[Q_i , Q_0 ]
\end{split}
\end{equation}
In the same fashion, the general form of the elements of $\Cov[\vec{\Delta}, \vec{\Delta}] $ is obtained:
\begin{equation}
\begin{split}
\Cov[\vec{\Delta}_i, \vec{\Delta}_j] =& \Cov[\hat Q_i(z^*_i) - \hat Q_i(z_i), \hat Q_j(z^*_j) - \hat Q_j(z_j)]\\
=& \Cov[\hat Q_i(z^*_i), \hat Q_j(z^*_j)] - \Cov[\hat Q_i(z^*_i), \hat Q_j(z_j)]\\
   & - \Cov[\hat Q_i(z_i), \hat Q_j(z^*_j)] + \Cov[\hat Q_i(z_i), \hat Q_j(z_j)]\\
=& \frac{N_{i* \cap j*}}{N_{i*}N_{j*}}\Cov[Q_i , Q_j ] - \frac{N_{i* \cap j}}{N_{i*}N_j}\Cov[Q_i , Q_j ]\\
   & - \frac{N_{i \cap j*}}{N_{i}N_{j*}}\Cov[Q_i , Q_j ] + \frac{N_{i \cap j}}{N_{i}N_j}\Cov[Q_i , Q_j ]\\
=& \left(\frac{N_{i* \cap j*}}{N_{i*}N_{j*}} - \frac{N_{i* \cap j}}{N_{i*}N_j}  - \frac{N_{i \cap j*}}{N_{i}N_{j*}}+ \frac{N_{i \cap j}}{N_{i}N_j} \right) \Cov[Q_i , Q_j ]
\end{split}
\end{equation}
Thus the form of the relationship between $\Cov[\vec{\Delta}, \vec{\Delta}]$, $\Cov[\vec{\Delta}, \hat Q_0]$, and $\mathcal{A}$ is thus:
\begin{align}
\Cov[\vec{\Delta}, \vec{\Delta}] &= \mathbf{G}(\mathcal{A}) \circ \mathbf{C} \label{eq:cov_delta_delta}\\
\Cov[\vec{\Delta}, \hat Q_0] &= \mathbf{g}(\mathcal{A}) \circ \mathbf{c} \label{eq:cov_delta_0}
\end{align}
with
\begin{align}
G_{ij} & = \frac{N_{i* \cap j*}}{N_{i*}N_{j*}} - \frac{N_{i* \cap j}}{N_{i*}N_j}  - \frac{N_{i \cap j*}}{N_{i}N_{j*}}+ \frac{N_{i \cap j}}{N_{i}N_j} \\
g_{i} & = \frac{N_{i* \cap 0}}{N_{i*}N_0} - \frac{N_{i \cap 0}}{N_{i}N_0}
\end{align}



Thus, assuming fixed model statistics, the variance of the ACV estimator with optimal weights becomes solely a function of sample allocation: 
\begin{equation}
\Var[\tilde{Q}^{\vec{\alpha}_{opt}}](\mathcal{A}) = \Var[\tilde Q(\vec{\alpha}_{opt}(\mathcal{A}), z, \mathcal{A})]  = \Var[\tilde Q^{\vec{\alpha}_{opt}}(z, \mathcal{A})]
\end{equation}



\subsubsection{ACV Optimization} 
Let $\vec{w} = \{w_0, ..., w_M\} $ represent the costs associated with the evaluation of each of the models.  The total cost of the ACV estimator is:
\begin{equation}
\tilde{w}(\vec{w}, \mathcal{A}) = w_0N_0 + \sum_{i=1}^M w_iN_{i^* \cup i}
\end{equation}
where $N_0$ is the number of model $0$ evaluations, \ie the number of samples in $z_0$.  $N_{i^* \cup i}$ is the number of model $i$ evaluations, \ie the number of samples in the union of $z_i^*$ and $z_i$.

The formal definition of the ACV optimization problem is here defined as the common case where an estimator for the expectation of a model $Q_0$ is sought with minimum variance given a set of models $\{Q_0, ..., Q_M\}$, costs $\vec{w}$, and a constraint on the total cost $\tilde{w}^*$. This simplifies to the identification of an optimal sample allocation $\mathcal{A}$:
\begin{equation}
\begin{split}
\min_{\mathcal{A}\in\mathbb{A}} & \Var[\tilde{Q}^{\vec{\alpha}_{opt}}](\mathcal{A})\\
\text{s.t.} &~\tilde{w}(\vec{w}, \mathcal{A}) \leq \tilde{w}^*
\end{split}
\label{eq:main_opt}
\end{equation}
where $\mathbb{A}$ is the set of all possible sample allocations.  Since $\mathcal{A}$ includes not only the number of samples in $z$ but also its relative division into $2M + 1$ subsets the domain of the optimization $\mathbb{A}$ is astronomically large.  In addition to the difficulty caused by the size of $\mathbb{A}$ an efficient means of parameterizing the domain is lacking.  This is compounded by the fact that calculation of $\vec{\alpha}_{opt}$ precludes a general analytical formula for the estimator variance.  

As illustrated by Gorodetsky et al. \ref{gorodetsky2018}, existing ACV estimators from the literature can be fit into the above framework.  These literature techniques include multifidelity MC (MFMC) [REFS], the recursive difference estimator associated with multi-level MC (MLMC) [REFS] and the several estimators formed in that work.  All of these methodologies approach the optimization in \eref{eq:main_opt} by restricting the optimization to subsets of $\mathbb{A}$ using an assumed sampling strategy\footnote{Note that standard MLMC also assumes values of $\alpha_i=1$ which is generally different than the $\vec{\alpha}_{opt}$}.  The sub-domains are smaller and easier to parameterize than $\mathbb{A}$; in the case of MLMC and MFMC the sub-domains are restricted sufficiently to permit analytical solutions of the optimization.  A key consequence of restricting optimization to sub-domains of $\mathbb{A}$ is that the optimal values found on the restricted domain are local minima and may not reflect the global minimum over $\mathbb{A}$.  

\subsubsection{The Sub-optimization Approach} 
A very practical approach to the optimization to break the problem into several sub-optimization problems.  The simplest case of performing the sub-optimization approach, which is common in practice, is to calculate the variance of multiple estimators like MLMC and MFMC then use the method with lowest variance.  In general terms the sub-optimization approach is
\begin{equation}
\min_{A_p \in \{1, \dots, P\}} \left(\begin{array}{rl}
\min\limits_{\mathcal{A}\in A_p} & \Var[\tilde{Q}^{\vec{\alpha}_{opt}}](\mathcal{A})\\
\text{s.t.} &~\tilde{w}(\vec{w}, \mathcal{A}) \leq \tilde{w}^*\\
\end{array}\right)
\label{eq:sub_opts}
\end{equation}
where $A_p \subset \mathbb{A}$ is one of a set of $P$ sub-domains.  As the effective optimization domain approaches $\mathbb{A}$ (\ie $A_1 \cup \dots \cup A_P \rightarrow \mathbb{A}$) the result of \eref{eq:sub_opts} approaches the result of \eref{eq:main_opt}; this of course assumes that the sub-optimizations find global minima in their restricted domains.  Since there is no reason to believe that sub-domains of current methods capture the global minimum, the intent of the current work is to enable the broadening of the effective optimization domain as much as possible.  With this aim, parametrically defined sub-domains are extensively explored in the current work.


\subsection{Automatic Model Selection}
The choice of which models to include in an ACV estimator has an effect on the resulting accuracy of the estimator.  This is due primarily to the fact that most estimators defined in the literature assume that all models must have samples allocated to them.  Since relaxing this constraint is not always practical within a sub-optimization, an alternative approach is to perform multiple sub-optimizations with differing subsets of models.  In this way sub-optimizations are parametrically defined based on subsets of $\{Q_0, Q_1, ..., Q_M\}$; thus, allowing for the number of samples allocated to a specific model to be 0 in the case that the model is not included in the sub-optimization.  Importantly, the high fidelity model must be a part of all model subsets in order for the estimators to remain unbiased.

A useful consequence of parametrically defining sub-optimizations based on model subsets is that a comparison is automatically made to the standard MC estimator (obtained when the model subset is  $\{Q_0\}$).  This comparison is standard for the ACV community.




\subsection{Generalized Recursion}
In the work of Gorodetsky et al.\ref{gorodetsky2018}, a sample allocation strategy, coined ACVKL, was developed that used the idea of tunable recursion to parametrically create sub-domains of $\mathbb{A}$ and corresponding sub-optimizations that were used in a sub-optimization scheme like \eref{eq:sub_opts}.  The motivating idea of the ACVKL estimator is that the first $K$ low fidelity models act as a control variate for the high fidelity model and the remaining models act as a control variate for estimating the mean of model $L$.  In this context, acting as a control variate implies that the first MC estimator of a model is maximally correlated with its target, \ie it shares the same set of samples.  More formally, if model $i$ is to act as a control variate for model $j$  then $z^*_i = z_j$.  

The notion of tunable recursion can be generalized further to include all possible ways of assigning models to act as control variates for other models.  In any sample allocation strategy of this type, there exists a zero-rooted acyclic tree which represents its recursion structure.  \fref{fig:recursion_trees} illustrates all the possible recursion structures for the case of four models.  Each recursion tree (and a corresponding sample allocation strategy) defines a sub-domain in $\mathbb{A}$ upon which to perform a sub-optimization.  Thus, when used in a sub-optimization scheme, the number of recursion trees enumerated relates to the size of the effective domain of the optimization.  The number of enumerated recursion trees also relates directly to the computational cost of performing the overall optimization.  This is not a reason for concern in most cases, especially since the sub-optimizations may be performed in parallel; however, due to the combinatorial nature of the recursion trees the number of possible trees increases rapidly with increased number of models (see \fref{fig:num_recursions}).   For this reason, it may be worth considering more limited recursion strategies.
\begin{figure}
\centering
\includegraphics[width=\textwidth]{figures/recursion_example.pdf}
\caption{All possible recusion trees with four models. $\raisebox{.5pt}{\textcircled{\raisebox{-.4pt} {\scriptsize $i$}}}\leftarrow$ \raisebox{.5pt}{\textcircled{\raisebox{-.4pt} {\scriptsize $j$}}} indicates that model $j$ acts as a control variate for model $i$.  The boxes represent the MR, SR, and KL recursion strategies.  Note that KL $\subset$ SR $\subset$ MR.  The list above each tree represents $\beta$ for that case.}
\label{fig:recursion_trees}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{figures/num_enum_vs_num_models.png}
\caption{Number of recursion trees as a function of the number of models.  The MR recursion strategy corresponds to all possible recursion trees.}
\label{fig:num_recursions}
\end{figure}

The KL recursion strategy discussed above limits the recursion trees to those with a depth less than or equal to two, in which model $i$ can be a control variate of model $j$ if $i> j$.  A slightly less restricted version of the KL recursion strategy contains all recursion trees with a depth less than or equal to 2, and assumes nothing about the ordering; this recursion strategy is henceforth called SR for single recursion.  The recursion strategy which contains all possible recursion trees regardless of size is henceforth called MR for multiple recursion.  Each of these recursion strategies is illustrated as a box in \fref{fig:recursion_trees}.  \fref{fig:num_recursions} shows that adding restrictions to the recursion trees drastically slows the explosion of possibilities with increasing numbers of models.

Every recursion tree can be represented by a mapping $\vec{\beta} \in \mathbb{R}^{M-1}$ from each low-fidelity model to the target of its control variate estimation, \ie $\beta_i = j$ implies $z^*_i = z_j$.  Note that the index of the $\vec{\beta}$ vector starts at 1, $i \in \{1, ..., M\}$, and contains values $j \in \{0, ..., M\}$.  As an example, the KL recursion strategy can be described with:
\begin{equation}
\beta^{KL} _i = \left\{\begin{array}{cl}
0 &: i \leq K\\
L &: i > K \\
\end{array}\right.
\end{equation}
The $\beta$ vector is illustrated for all the four-model recursion trees in \fref{fig:recursion_trees}.

\subsubsection{Generalized Multifidelity (GMF) Estimators}
The last two ingredients to a generalized recursion sub-optimization are the development of (1) a variance calculation based on the recursion structure and (2) a means to calculate the number model evaluations $N_0, N_{i^* \cup i}$ for the total cost calculation.  The multifidelity sample allocation strategy used in MFMC and ACVMF is used for this purpose.  In this sample allocation strategy all subsets of $z$ are defined based on their size $N_i$ and include the first $N_i$ samples of $z$: \ie $z_i = \{z^{(1)}, \dots, z^{(N_i)} \}$.  

Based on the multifidelity sample allocation strategy and the definition of $\beta$, the elements of $\mathbf{G}$ and $\mathbf{g}$ are defined as follows:
\begin{equation}
\begin{split}
G_{ij}^{GMF} & = \frac{N_{i* \cap j*}}{N_{i*}N_{j*}} - \frac{N_{i* \cap j}}{N_{i*}N_j}  - \frac{N_{i \cap j*}}{N_{i}N_{j*}}+ \frac{N_{i \cap j}}{N_{i}N_j} \\
& = \frac{N_{\beta_i \cap \beta_j}}{N_{\beta_i}N_{\beta_j}} - \frac{N_{\beta_i \cap j}}{N_{\beta_i}N_j}  - \frac{N_{i \cap \beta_j}}{N_{i}N_{\beta_j}}+ \frac{N_{i \cap j}}{N_{i}N_j} \\
& = \frac{\min(N_{\beta_i}, N_{\beta_j})}{N_{\beta_i}N_{\beta_j}} - \frac{\min(N_{\beta_i}, N_j)}{N_{\beta_i}N_j}  - \frac{\min(N_i, N_{\beta_j})}{N_{i}N_{\beta_j}} + \frac{\min(N_i,  N_j)}{N_{i}N_j} 
\end{split}
\end{equation}
\begin{equation}
\begin{split}
g_{i}^{GMF} & = \frac{N_{i* \cap 0}}{N_{i*}N_0} - \frac{N_{i \cap 0}}{N_{i}N_0}\\
& = \frac{N_{\beta_i \cap 0}}{N_{\beta_i}N_0} - \frac{N_{i \cap 0}}{N_{i}N_0}\\
& = \frac{\min(N_{\beta_i},N_0)}{N_{\beta_i}N_0} - \frac{\min(N_i, N_0)}{N_{i}N_0}\\
\end{split}
\end{equation}
where $N_{\beta_i} = N_k$ for $\beta_i = k$.  From here \eqs{eq:cov_delta_delta}{eq:cov_delta_0} can be used in conjunction with \eref{eq:acv_est_var} to produce the generalized multifidelity (GMF) estimator variance as a function of $\vec{N} = \{N_0, \dots, N_M\}$ and $\vec{\beta}$.

Analogously, the number of model evaluations are $N_{i^* \cup i} = \max(N_{\beta_i}, N_i)$ for the GMF estimator.  Again noting that they are a function of $\vec{N}$ and $\vec{\beta}$.

The resulting sub-optimization scheme is
\begin{equation}
\min_{\vec{\beta}} \left(\begin{array}{rl}
\min\limits_{\vec{N}} & \Var[\tilde{Q}^{GMF}](\vec{N}, \vec{\beta})\\
\text{s.t.} &~\tilde{w}(\vec{N}, \vec{\beta}) \leq \tilde{w}^*\\
\end{array}\right)
\label{eq:sub_opts}
\end{equation}
Where each sub-optimization is performed on variables $\vec{N}$ associated with the sizes of the subsets of $z$.

A schematic view of the sample allocation associated with the GMF estimator is shown in \fref{fig:gmf_diagram}.  It also illustrates how MFMC and ACVMF are equivalent to GMF with specific values of $\vec{\beta}$.  The $\vec{\beta}$ associated with fully recursive structure of MFMC is $\{0, 1,\dots, M-1\}$.  The $\vec{\beta}$ associated with ACVMF is $\vec{0}$.  

\begin{figure}
\centering
\small
\setlength\tabcolsep{1.5pt}

\begin{subfigure}{.5\textwidth}
  \centering
\begin{tabular}{ccccccc}
$z_0$ & $z_{1*}$ & $z_1$& $z_{2*}$ & $z_2$& $z_{3*}$ & $z_3$ \\
\cellcolor{red}&\cellcolor{orange}&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
$N_0$&\cellcolor{orange}&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&$N_{\beta_1}$&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&&$N_1$&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&&&$N_{\beta_2}$&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&&&&$N_2$&\cellcolor{magenta}&\cellcolor{black}\\
&&&&&$N_{\beta_3}$&\cellcolor{black}\\
&&&&&&$N_3$
\end{tabular}

(a) Generalized Multifidelity (GMF)
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
\begin{tabular}{ccccccc}
$z_0$ & $z_{1*}$ & $z_1$& $z_{2*}$ & $z_2$& $z_{3*}$ & $z_3$ \\
\cellcolor{red}&\cellcolor{orange}&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
$N_0$&$N_0$&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&&$N_1$&$N_1$&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
&&&&$N_2$&$N_2$&\cellcolor{black}\\
&&&&&&$N_3$
\end{tabular}

(b) MFMC, $\vec{\beta} = \{0, 1, 2 \}$

\vspace{2em}
\begin{tabular}{ccccccc}
$z_0$ & $z_{1*}$ & $z_1$& $z_{2*}$ & $z_2$& $z_{3*}$ & $z_3$ \\
\cellcolor{red}&\cellcolor{orange}&\cellcolor{yellow}&\cellcolor{green}&\cellcolor{blue}&\cellcolor{magenta}&\cellcolor{black}\\
$N_0$&$N_0$&\cellcolor{yellow}&$N_0$&\cellcolor{blue}&$N_0$&\cellcolor{black}\\
&&$N_1$&&\cellcolor{blue}&&\cellcolor{black}\\
&&&&$N_2$&&\cellcolor{black}\\
&&&&&&$N_3$
\end{tabular}

(c) ACVMF, $\vec{\beta} = \{0, 0, 0 \}$
\end{subfigure}
\caption{Multifidelity sample allocations for four models with sampling strategies (a) GMF, (b) MFMC, and (c) ACVMF.}
\label{fig:gmf_diagram}
\end{figure}


\subsubsection{Generalized Recursive Difference (GRD) Estimators}
In the same vein as the GMF estimators, the recursive difference sample allocation strategy associated MLMC and WRDIFF can be generalized for any recursion structure.  In the recursive difference sample allocation strategy, the subsets $z_i$ of $z$ are disjoint (\ie independent). The elements of $\mathbf{G}$ and $\mathbf{g}$ for the generalized recursive difference (GRD) estimator are:
\begin{equation}
\begin{split}
G_{ij}^{GRD} =&  \left(\begin{array}{rl} \frac{1}{N_{\beta_i}} &: \beta_i=\beta_j\\ 0&: \beta_i \neq \beta_j\end{array}\right) 
- \left(\begin{array}{rl} \frac{1}{N_{\beta_i}} &: \beta_i=j\\ 0&: \beta_i \neq j\end{array}\right) \\
&- \left(\begin{array}{rl} \frac{1}{N_i} &: i=\beta_j\\ 0&: i \neq \beta_j\end{array}\right) 
+ \left(\begin{array}{rl} \frac{1}{N_i} &: i=j\\ 0&: i \neq j\end{array}\right) 
\end{split}
\end{equation}
\begin{equation}
\begin{split}
g_{i}^{GRD} =& \left(\begin{array}{rl} \frac{1}{N_{\beta_i}} &: \beta_i=0\\ 0&: \beta_i \neq 0\end{array}\right)
\end{split}
\end{equation}
The number of evaluations of model $i$ with GRD are $N_{i^* \cup i} = N_{\beta_i} + N_i$.  As with the GMF estimator the sub-optimization problem boils down to optimizations of $\vec{N}$ given $\vec{\beta}$:
\begin{equation}
\min_{\vec{\beta}} \left(\begin{array}{rl}
\min\limits_{\vec{N}} & \Var[\tilde{Q}^{GRD}](\vec{N}, \vec{\beta})\\
\text{s.t.} &~\tilde{w}(\vec{N}, \vec{\beta}) \leq \tilde{w}^*\\
\end{array}\right)
\label{eq:sub_opts}
\end{equation}
Schematics of sample allocations for the GRD estimator are shown in \fref{fig:grd_diagram} in addition to two examples of the estimator with given $\beta$.  The WRDIFF estimator is an instance of the GRD estimator with $\vec{\beta} = \{0, 1,\dots, M-1\}$.

\begin{figure}
\centering
\small
\setlength\tabcolsep{1.5pt}

\begin{subfigure}{.5\textwidth}
  \centering
\begin{tabular}{ccccccc}
$z_0$ & $z_{1*}$ & $z_1$& $z_{2*}$ & $z_2$& $z_{3*}$ & $z_3$ \\
\cellcolor{red}&&&&&&\\
$N_0$&\cellcolor{orange} $\updownarrow$&&&&&\\
&$N_{\beta_1}$&\cellcolor{yellow}&&&&\\
&&$N_1$&\cellcolor{green}$\updownarrow$&&&\\
&&&$N_{\beta_2}$&\cellcolor{blue}&&\\
&&&&$N_2$&\cellcolor{magenta}$\updownarrow$&\\
&&&&&$N_{\beta_3}$&\cellcolor{black}\\
&&&&&&$N_3$
\end{tabular}

(a) Generalized Recursive Difference (GRD)
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
\begin{tabular}{ccccccc}
$z_0$ & $z_{1*}$ & $z_1$& $z_{2*}$ & $z_2$& $z_{3*}$ & $z_3$ \\
\cellcolor{red}&\cellcolor{orange}&&&&&\\
$N_0$&$N_0$&\cellcolor{yellow}&\cellcolor{green}&&&\\
&&$N_1$&$N_1$&\cellcolor{blue}&\cellcolor{magenta}&\\
&&&&$N_2$&$N_2$&\cellcolor{black}\\
&&&&&&$N_3$
\end{tabular}

(b) WRDIFF, $\vec{\beta} = \{0, 1, 2 \}$
\end{subfigure}
\caption{Recursive difference sample allocations for four models with sampling strategies (a) GMF and (b) WRDIFF.  The arrows indicate that the $z_{i*}$ samples will move based on the values of $\vec{\beta}$}
\label{fig:gmf_diagram}
\end{figure}
It is also possible to generalize the independent sample strategy associated with ACVIS, which is very similar to the GRD.  This generalization was performed, but is left out here because the variances of the generalized independent samples strategy rarely deviated appreciably from  GMF.

 


